ATLAS: A Self-Supervised and Cross-Stage Netlist Power Model for Fine-Grained Time-Based Layout Power Analysis

Accurate power prediction in VLSI design is crucial for effective power optimization, especially as designs get transformed from gate-level netlist to layout stages. However, traditional accurate power simulation requires time-consuming back-end processing and simulation steps, which significantly impede design optimization. To address this, we propose ATLAS, which can predict the ultimate time-based layout power for any new design in the gate-level netlist. To the best of our knowledge, ATLAS is the first work that supports both time-based power simulation and general cross-design power modeling. It achieves such general time-based power modeling by proposing a new pre-training and fine-tuning paradigm customized for circuit power. Targeting golden per-cycle layout power from commercial tools, our ATLAS achieves the mean absolute percentage error (MAPE) of only 0.58%, 0.45%, and 5.12% for the clock tree, register, and combinational power groups, respectively, without any layout information. Overall, the MAPE for the total power of the entire design is <1%, and the inference speed of a workload is significantly faster than the standard flow of commercial tools.

==> section/2-preliminaries.tex <==


\section{Preliminaries}\label{sec:pre}


%\subsection{Power Modeling Solution}
%Table~\ref{tbl:prior work} shows the comparison between our ATLAS with previous ML-based power modeling methods. 





\begin{table}[!t]
\centering
%that are most relevant to this proposal.} % \footnote{GRANNITE~\cite{zhang2020grannite} estimates toggle rate instead of power.}
 \renewcommand{\arraystretch}{1.2}
 \resizebox{.5\textwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|}
\hline 
Power Models &
  \begin{tabular}[c]{@{}c@{}}Applied \\ Stage\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Use\\ Workload\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Time- \\ Based\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Cross- \\ Design\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Target \\ Layout\end{tabular} \\ \hline\hline
\begin{tabular}[c]{@{}c@{}}PRIMAL [DAC'20]~\cite{zhou2019primal} \\ APOLLO [MICRO'21]~\cite{xie2021apollo}\end{tabular} &   \multirow{4}{*}{RTL} &  Yes &  Yes &  No &  \multirow{4}{*}{No} \\ \cline{1-1} \cline{3-5}
\begin{tabular}[c]{@{}c@{}}SNS [ISCA'22]~\cite{xu2022sns}\\SNS V2 [MICRO'23]~\cite{xu2023fast}\end{tabular} &   &  No &  \multirow{3}{*}{No} &  \multirow{3}{*}{Yes} &   
\\ \cline{3-3}  
MasterRTL [ICCAD'23]~\cite{fang2023masterrtl}&                      & Yes          &                     &                      &                     \\ \cline{1-3} \cline{6-6} 
PowPredicCT [DAC'24]~\cite{du2024powpredi} &  Layout &  No &   &   &  Yes \\ \hline\hline
ATLAS &  Netlist &  \textbf{Yes} &  \textbf{Yes} &  \textbf{Yes} &  \textbf{Yes} \\ \hline
\end{tabular}
}
\begin{tablenotes}\footnotesize
\item $^*$GRANNITE~\cite{zhang2020grannite} estimates toggle rate instead of power, thus not listed in the table. It is neither time-based nor targeting layout. 
\end{tablenotes} 
\caption{Summary of representative ML-based power models.} 
\label{tbl:prior work}
 \vspace{-.2in}
\end{table}



%\subsubsection{Time-based but not Cross-design}
%\label{sec:time-no-cross}

%An important type of work is time-based but not cross-design. As Table~\ref{tbl:prior work} shows, representative works include 






%in this work, a cross-design solution is required, making the task much more challenging.  
%Compared with the early architecture level, power modeling is generally more accurate at the RTL or netlist stage, when sufficient design details become available. For this type of work, early works~\cite{bogliolo2000regression, wu1998cycle, ye2000design} were proposed 20 years ago. They construct macro-models to abstract power estimations for small circuit modules with thousands of gates. In recent years, machine learning (ML) techniques are exploited~\cite{zhou2019primal, xie2021apollo}. 

%PRIMAL~\cite{zhou2019primal} predicts per-cycle power by processing transitions of all registers with multiple ML methods, including both the convolutional neural network (CNN) and principle component analysis (PCA) plus linear model. APOLLO~\cite{xie2021apollo} predicts per-cycle power by selecting the most power-correlated signals with a pruning method named MCP. If we inspect PRIMAL~\cite{zhou2019primal} and APOLLO~\cite{xie2021apollo} in detail, their overall problem formulation and setup are similar and straightforward.  Given all register signals or RTL signals as input candidates, the key point is to avoid overfitting. Despite targeting the most challenging per-cycle temporal granularity, their overall accuracy values are very high (error $<$ 10\%). 


%\subsubsection{Cross-design but not Time-based}
%\label{sec:cross-no-time}
%Different from works in Section~\ref{sec:time-no-cross}, another type of work at the RTL stage is the opposite, they are cross-design but not time-based. Instead of directly fitting the type-I model in Section~\ref{sec:time-no-cross}, these works have to capture detailed design information of each unknown test design. Representative early explorations include Sengupta et al.~\cite{sengupta2022good} and SNS~\cite{xu2022sns} published in 2022. They first convert design RTL to representations such as the abstract syntax tree (AST), and then evaluate design timing and power either based on all register trees~\cite{sengupta2022good} or randomly sampled paths~\cite{xu2022sns}. Subsequent works include MasterRTL~\cite{fang2023masterrtl} and SNS-V2~\cite{xu2023fast} in 2023. They partition the design into multiple parts and estimate the power in each part based on its scale and toggle information.  


%However, completely cross-design prediction is highly challenging. As a result, all these works~\cite{sengupta2022good, xu2022sns, xu2023fast, fang2023masterrtl} only target average power only, instead of modeling time-based power. Some works even modeled the vectorless power number without specific testbenches. Even in this case, the overall model accuracy is not high. The obvious difficulty of this type of work teaches us a lesson: for higher accuracy, we better modify/tune the power model for each given test design.    

%In addition to the works~\cite{sengupta2022good, xu2022sns, xu2023fast, fang2023masterrtl} mentioned above, GRANNITE ~\cite{zhang2020grannite} is a very special method. Although it is very commonly categorized as a power model and a follow-up work of PRIMAL~\cite{zhou2019primal}, largely due to common authors from NVIDIA, actually it does not focus on the power simulation part at all. 
%After inspecting state-of-the-art works in both Section~\ref{sec:time-no-cross} and~\ref{sec:cross-no-time}, we can easily notice that very few works achieve time-based and cross-design solutions at the same time. However, this project raises high requirements in multiple aspects, including 1) cross-design, 2) time-based, 3) high-accuracy, and 4) targeting very large-scale designs. We will introduce our plan and experience in developing both cross-design and time-based solutions in Section~\ref{sec:method1}.

\subsection{Netlist Representation Learning}
Graph Neural Networks (GNNs)~\cite{xu2018how} have consistently been regarded as effective models for learning from graph-structured data. A netlist, by its nature, is a type of graph where instances represent the nodes and the connections between them constitute the vertices. This has led to the development of numerous GNN models specifically designed for representation learning~\cite{Deepgate1,deepgate2,functionDAC2022}. 

While GNNs are a good choice for circuit learning, they exhibit limitations in inferring large-scale circuit graphs. The graph embeddings generated at each layer require substantial storage for neighborhood information, resulting in significant resource consumption during training. Moreover, GNNs perform well when inferring global properties but struggle with local attributes, such as critical paths, which are crucial for circuit inference. Consequently, GNNs are not well-suited for inference tasks involving large-scale circuits.



Transformers, with their unique self-attention mechanism, effectively capture long-range dependencies between nodes. To enhance the capture of local information in graphs, integrating Transformers as foundational encoders with GNNs has proven to be an excellent approach~\cite{wu2023difformer,Wu2021GraphTrans,NodeFormer}. Furthermore, Transformers allow for the parallel processing of all nodes in a graph, making them more efficient for handling large-scale graphs.

\question{Although Graph Transformers demonstrate strong performance on small graphs, they face challenges when dealing with larger graphs. Because of the global all-pair attention mechanism in Transformers, the time and space complexity will scale quadratically with the number of nodes. Additionally, as the number of layers increases, the size of the computation graph expands exponentially.}

\subsection{Netlist Contrastive Learning}
Contrastive Learning is a self-supervised learning method aimed at learning effective representations of data by comparing the similarities and differences between samples. This approach typically involves constructing pairs of positive samples (similar samples) and negative samples (dissimilar samples) during training, such that similar samples are brought closer together in the representation space, while dissimilar samples are pushed further apart.

These papers~\cite{Deepgate1, deepgate2, functionDAC2022} have focused on learning the representation similarities of different circuits on very small graphs (consisting of a few or several dozen nodes) and have not been extended to real chips (with millions of nodes or more). Furthermore, these works have only pre-trained a general task for downstream applications and have not specifically addressed pre-training for power estimation. As a result, when using those pre-train models to do finetuning, the performance of per-cycle level power prediction for real chips is suboptimal.





\section{Problem Formulation}
\label{sec:problem}
\textbf{Problem: }Given a synthesized netlist derived from a real chip design with over one hundred thousand cells, the objective is to predict the per-cycle power consumption after placement and routing under real workloads. Our model must learn the netlist transformation that occurs from synthesis to placement and routing, as well as the toggling behavior of all instance ports within the netlist across different cycles.

Cross-stage power prediction, especially for per-cycle power estimation, has long been a challenging task. To address this gap, we propose ATLAS, the first framework designed to predict the fine-grained per-cycle power consumption of post-P\&R netlists with real workloads starting from the gate-level netlists.

\iffalse

\textbf{Problem 1}: Given a gate-level netlist ${N_g}$, we aim to extract a set of non-overlapping sub-netlists ${N_g\in\{g_1,g_2,...,g_i\}}$ that, when concatenated, fully represent the entire netlist. After the placement and routing, ${N_g}$ generates a corresponding post-layout netlist ${N_p}$, which will similarly yield a set of sub-netlists ${N_p\in\{p_1,p_2,...,p_i\}}$. The objective is to align the sets ${\{g_1,g_2,...,g_i\}}$ and ${\{p_1,p_2,...,p_i\}}$ within the framework of contrastive learning ($f_{C\!L}$).This alignment aims to ensure that corresponding sub-netlists from the gate-level representation and the post-layout representation are effectively matched, thereby generating an embedding ${E_{g_i}}$ for ${\{g_i\}}$ and ${E_{p_i}}$ for ${\{p_i\}}$.  By maximizing the similarity between ${E_{g_i}}$ and ${E_{p_i}}$, the model can accurately capture the differences of netlist reconstruction.%enhancing the learning process  between related pairs while minimizing the similarity between unrelated pairs.
\begin{equation}
f_{\text{CL}}({\{g_i\}} \& {\{p_i\}}) \rightarrow max({Similarity(E_{g_i},E_{p_i}))} 
\label{eq:fcl}
\end{equation}

% No one has ever predicted the per-cycle power of the post-placement and routing netlist under real workloads starting from the gate level. Therefore, our objective is to be the first to accomplish this task, utilizing a gate-level netlist derived from a real chip containing over one hundred thousand gates. We divide our problem into the following two parts:

% \textbf{Problem 1}: We require a novel Transformer-based GNN to serve as the encoder for our self-supervised Contrastive Learning model($f_{C\!L}$). This encoder must be capable of handling large graphs while consuming significantly fewer resources than previous implementations. Our model needs to learn the transformations that occur in the netlist from gate level to post-placement and routing, including netlist reconstruction and CTS, the latter of which is completely absent at the gate level. We represent the gate-level netlist as \emph{Ori\_N} and the post-layout netlist as \emph{PR\_N}. Our goal is to align the representations of \emph{Ori\_N} and \emph{PR\_N} as closely as possible in the latent space, thereby generating an embedding $E_{O}$ for \emph{Ori\_N} that accurately represents the netlist reconstruction and CTS. We denote this process as follows:
% \begin{equation}
% \text{pre-train}\left(f_{\text{CL}}(\emph{Ori\_N} \& \emph{PR\_N})\right) \rightarrow E_{\mathcal{O}} 
% \end{equation}

\textbf{Problem 2}: To predict per-cycle power, 
% our model must also learn how all instance ports within the netlist toggle across different cycles and how toggles propagate between instances. 
our model must capture the circuit's operational states at different timestamps, recognizing that the toggle activities of various cells vary under real workloads. 
We employ a systematic method to extract dynamic toggle information at discrete timestamps ${t_{\theta}}$.
To enhance learning, we introduce a mechanism that randomly masks the toggle information of specific cells, allowing the model to effectively learn toggle propagation and improve its understanding of power consumption.
\begin{equation}
\left\{
\begin{aligned}
&{N_g} \rightarrow {\{N_{g}(t_{0}),N_{g}(t_{1}),...,N_{g}(t_{\theta})\}} \\
&{N_p} \rightarrow {\{N_{p}(t_{0}),N_{p}(t_{1}),...,N_{p}(t_{\theta})\}} \\
\end{aligned}
\right.
\label{eq:theta}
\end{equation}

\fi


==> section/5-discussion.tex <==

\section{Discussion} \label{sec:disc}


